Bayesian model selection for unsupervised image deconvolution with structured Gaussian priors

This paper considers the objective comparison of stochastic models to solve inverse problems, more specifically image restoration. Most often, model comparison is addressed in a supervised manner, that can be time-consuming and partly arbitrary. Here we adopt an unsupervised Bayesian approach and objectively compare the models based on their posterior probabilities, directly from the data without ground truth available. The probabilities depend on the marginal likelihood or "evidence" of the models and we resort to the Chib approach including a Gibbs sampler. We focus on the family of Gaussian models with circulant covariances and unknown hyperparameters, and compare different types of covariance matrices for the image and noise.

==> abrege.tex <==
% TEX 7(ascii) bits
%
% ABREGE.tex
% LaTeX document
% Author: J.I. 
% Date  : Juillet 1996
%
% Raccourcis d'expressions très usitées
%
% Derniere modif le 10-07-96
%
%
% ==> OK, JFG -- 26/04/2010
%

% Raccourci pour \XS
\def\XS{\xspace}

%%%%%%%%%%%%%%%%%%% Pour definir nouvelle commande de changement de taille
\RequirePackage{ifthen}
\RequirePackage{calc}

\newcommand{\taille}[1][\scad]{%
\ifthenelse{#1 = -5}{}{}%
\ifthenelse{#1 = -4}{\tiny}{}%
\ifthenelse{#1 = -3}{\scriptsize}{}%
\ifthenelse{#1 = -2}{\footnotesize}{}%
\ifthenelse{#1 = -1}{\small}{}%
\ifthenelse{#1 = 0}{\normalsize}{}%
\ifthenelse{#1 = 1}{\large}{}%
\ifthenelse{#1 = 2}{\Large}{}%
\ifthenelse{#1 = 3}{\LARGE}{}%
\ifthenelse{#1 = 4}{\huge}{}%
\ifthenelse{#1 = 5}{\Huge}{}}

\newboolean{@serif}
\setboolean{@serif}{true}
\def\scad{-5} % scadefaultsize

\newcounter{taille}
\newcommand{\sca}[2][\scad]{\setcounter{taille}{#1}%
  \ifthenelse{\boolean{@serif}}
  {{\taille[\thetaille]\textsc{#2}}}
  {\setcounter{taille}{\value{taille}-1}{\uppercase{\taille[\thetaille]#2}}}}


%%% RACCOURCIS DIVERS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Mise en commentaire rapide !
	\def\Rem#1{}                    % rem{bla bla bla}

% References automatiquement entre parenthese
	%\def\reff#1{\XS(\ref{#1})}
	%\def\refs#1{section~\ref{#1}}
	%\def\refS#1{Section~\ref{#1}}

% Nettoyage
	%\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}  

% Numéro (pour biblio)
	\def\numero{n°}
	\def\Numero{N°}

% Majuscules
	\def\UP#1{\uppercase{#1}}       % majuscules
	\def\up#1{\uppercase{#1}}       % majuscules

% References automatiquement entre parenthese
 \def\reff#1{\XS(\ref{#1})}
 %\def\refs#1{section~\ref{#1}}
 %\def\refS#1{Section~\ref{#1}}

%%% RACCOURCIS d'italique, locutions,... %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\adhoc{\textit{ad hoc}\XS}
\def\apost{\textit{a posteriori}\XS}
\def\Apost{\textit{A posteriori}\XS}
\def\APost{\textit{A Posteriori}\XS}
\def\post{\textit{posterior}\XS}
\def\Post{\textit{Posterior}\XS}
\def\afortio{\textit{a fortiori}\XS}
\def\Afortio{\textit{A fortiori}\XS}
\def\aprio{\textit{a priori}\XS}
\def\Aprio{\textit{A priori}\XS}
\def\Cad{C'est-à-dire\XS}
\def\cad{c'est-à-dire\XS}
\def\Cpq{C'est pourquoi\XS}
\def\cpq{c'est pourquoi\XS}
\def\coeur{c{\oe}ur\XS}
\def\cf{\textit{cf.}\XS}
\def\eg{\textit{e.g.,}\XS}
\def\etal{\textit{et al.}\XS}
%\def\etc{\textit{etc\dots}\XS}
\def\etcoll{{\textit et coll.}\XS}
\def\idem{\textit{idem}\XS}
\def\ie{\textit{i.e.,}\XS}
\def\iid{i.i.d.\XS}
\def\infine{\textit{in fine}\XS}
\def\insit{\textit{in situ}\XS}
\def\inviv{\textit{in vivo}\XS}
\def\oeuvre{{\oe}uvre\XS}
\def\oeuvres{{\oe}uvres\XS}
\def\oeil{{\oe}il\XS}
\def\recto{\textit{recto}\XS}
\def\Toeplitz{T{\oe}plitz\XS}
\def\vav{vis-à-vis\XS}
\def\via{\textit{via}\XS}
\def\vic{\textit{vice-versa}\XS}
\def\verso{\textit{verso}\XS}
\def\vs{\textit{vs}\XS}
\def\versus{\textit{versus}\XS}
\def\ssi{\textit{si et seulement si}\XS}
\def\strsen{\textit{stricto sensu}\XS}
\def\wrt{w.r.t.\XS}

\def\ier{$^{\text{\small er}}$\XS}
\def\iere{$^{\text{\small re}}$\XS}
\def\ieme{$^{\text{\small e}}$\XS}

\def\primo{\ensuremath{1^{\oD}}\XS}
\def\secundo{\ensuremath{2^{\oD}}\XS}
\def\tertio{\ensuremath{3^{\oD}}\XS}
\def\quatro{\ensuremath{4^{\oD}}\XS}

	\def\MALDI{Matrix-Assisted Laser Desorption/Ionisation\XS}
	\newcommand{\maldi}[1][\scad]{\sca[#1]{maldi}\XS}

	\def\BHIPRO{Bayesian Hierarchical Inversion in Proteomics\XS}
	\newcommand{\bhipro}[1][\scad]{\sca[#1]{bhi-pro}\XS}

	\def\BNPSI{Bayesian Non-Parametreic in Signal-Image\XS}
	\newcommand{\bnpsi}[1][\scad]{\sca[#1]{bnp-si}\XS}

%%% ACRONYMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Divers 
	\newcommand{\art}[1][\scad]{\sca[#1]{art}\XS}
	\newcommand{\cnd}[1][\scad]{\sca[#1]{cnd}\XS}
	\newcommand{\ndt}[1][\scad]{\sca[#1]{ndt}\XS}
	\newcommand{\gnc}[1][\scad]{\sca[#1]{gnc}\XS}
	\newcommand{\mfa}[1][\scad]{\sca[#1]{mfa}\XS}
	\newcommand{\map}[1][\scad]{\sca[#1]{map}\XS}

	\newcommand{\icm}[1][\scad]{\sca[#1]{icm}\XS}
	\newcommand{\icd}[1][\scad]{\sca[#1]{icd}\XS}
	\newcommand{\rsb}[1][\scad]{\sca[#1]{rsb}\XS}
	\newcommand{\snr}[1][\scad]{\sca[#1]{snr}\XS}
	\newcommand{\fft}[1][\scad]{\sca[#1]{fft}\XS}
	\newcommand{\fftdd}[1][\scad]{\sca[#1]{fft-2d}\XS}
	\newcommand{\ifft}[1][\scad]{\sca[#1]{ifft}\XS}
	\newcommand{\dsp}[1][\scad]{\sca[#1]{dsp}\XS}

	\newcommand{\dess}[1][\scad]{\sca[#1]{dess}\XS}
	\newcommand{\dea}[1][\scad]{\sca[#1]{dea}\XS}
	\newcommand{\deug}[1][\scad]{\sca[#1]{deug}\XS}
	\newcommand{\deust}[1][\scad]{\sca[#1]{deust}\XS}
	\newcommand{\iut}[1][\scad]{\sca[#1]{iut}\XS}
	\newcommand{\iup}[1][\scad]{\sca[#1]{iup}\XS}
	\newcommand{\ects}[1][\scad]{\sca[#1]{ects}\XS}

	\newcommand{\ufr}[1][\scad]{\sca[#1]{ufr}\XS}
	\newcommand{\uf}[1][\scad]{\sca[#1]{uf}\XS}
	\newcommand{\upr}[1][\scad]{\sca[#1]{upr}\XS}

	\newcommand{\gbm}[1][\scad]{\sca[#1]{gbm}\XS}
	\newcommand{\irmf}[1][\scad]{\sca[#1]{irm-f}\XS}
	\newcommand{\irm}[1][\scad]{\sca[#1]{irm}\XS}
	\newcommand{\rmn}[1][\scad]{\sca[#1]{rmn}\XS}
	\newcommand{\eeg}[1][\scad]{\sca[#1]{eeg}\XS}
	\newcommand{\meg}[1][\scad]{\sca[#1]{meg}\XS}


% Transformées
	\newcommand{\tf}[1][\scad]{\sca[#1]{tf}\XS}
	%\newcommand{\sf}[1][\scad]{\sca[#1]{sf}\XS}
	\def\sf{\textsc{sf}\XS}
	\newcommand{\tl}[1][\scad]{\sca[#1]{tl}\XS}
	\newcommand{\tz}[1][\scad]{\sca[#1]{tz}\XS}
	\newcommand{\tpsc}[1][\scad]{\sca[#1]{tc}\XS}
	\newcommand{\tpsd}[1][\scad]{\sca[#1]{td}\XS}

% Operating Systemes 
	\newcommand{\linux}[1][\scad]{\sca[#1]{Linux}\XS}
	\newcommand{\unix}[1][\scad]{\sca[#1]{Unix}\XS}
	\newcommand{\msdos}[1][\scad]{\sca[#1]{msdos}\XS}
	\newcommand{\sunos}[1][\scad]{\sca[#1]{Sunos}\XS}
	\newcommand{\hupux}[1][\scad]{\sca[#1]{hp-ux}\XS}
	\newcommand{\vms}[1][\scad]{\sca[#1]{vms}\XS}
	\newcommand{\solaris}[1][\scad]{\sca[#1]{Solaris}\XS}
	\newcommand{\winnt}[1][\scad]{\sca[#1]{Windows-nt}\XS}
	\newcommand{\vmware}[1][\scad]{\sca[#1]{vmware}\XS}
	\newcommand{\win}[1][\scad]{\sca[#1]{Windows}\XS}

% Calcul scientifique
	\newcommand{\labview}[1][\scad]{\sca[#1]{Labview}\XS}
	\newcommand{\matlab}[1][\scad]{\sca[#1]{Matlab}\XS}
	\newcommand{\maple}[1][\scad]{\sca[#1]{Maple}\XS}
	\newcommand{\mathe}[1][\scad]{\sca[#1]{Mathematica}\XS}
	\newcommand{\idl}[1][\scad]{\sca[#1]{Idl}\XS}

% Langages
	\newcommand{\cmex}[1][\scad]{\sca[#1]{Cmex}\XS}
	\newcommand{\pascal}[1][\scad]{\sca[#1]{Pascal}\XS}
	\newcommand{\java}[1][\scad]{\sca[#1]{Java}\XS}
	\newcommand{\lisp}[1][\scad]{\sca[#1]{Lisp}\XS}
	\newcommand{\forts}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 77}\XS}
	\newcommand{\fortq}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 90}\XS}
	\newcommand{\ada}[1][\scad]{\sca[#1]{Ada}\XS}
	\newcommand{\eiffel}[1][\scad]{\sca[#1]{Eiffel}\XS}
	\newcommand{\tcsh}[1][\scad]{\sca[#1]{tcsh}\XS}
	\newcommand{\bash}[1][\scad]{\sca[#1]{bash}\XS}
	\newcommand{\lgc}[1][\scad]{\sca[#1]{C}\XS}
	\newcommand{\cpp}[1][\scad]{\sca[#1]{C}{\footnotesize ++}\XS}

% Congres
	\newcommand{\gretsi}[1][\scad]{\sca[#1]{gretsi}\XS}
	\newcommand{\maxent}[1][\scad]{\sca[#1]{maxent}\XS}
	\newcommand{\icip}[1][\scad]{\sca[#1]{icip}\XS}
	\newcommand{\icassp}[1][\scad]{\sca[#1]{icassp}\XS}
	\newcommand{\spie}[1][\scad]{\sca[#1]{spie}\XS}
	%\newcommand{\gdr}[1][\scad]{\sca[#1]{gdr--prc~isis}\XS}
	\newcommand{\gdr}[1][\scad]{\sca[#1]{gdr~isis}\XS}
	\newcommand{\rfia}[1][\scad]{\sca[#1]{rfia}\XS}
	\newcommand{\eusipco}[1][\scad]{\sca[#1]{eusipco}\XS}

% Restes
	\newcommand{\leti}[1][\scad]{\sca[#1]{leti}\XS}
	\newcommand{\cesta}[1][\scad]{\sca[#1]{cesta}\XS}
	\newcommand{\minatec}[1][\scad]{\sca[#1]{minatec}\XS}
	\newcommand{\stic}[1][\scad]{\sca[#1]{stic}\XS}
	\newcommand{\pc}[1][\scad]{\sca[#1]{pc}\XS}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ajout de famouss.tex
% modif le 25/5/2000 Phiphi
% GPInuts - Famous people - VIP
%
\newcommand{\beaunom}[4][0]{{\taille[#1]#2 \uppercase{#3}}{\sca[#1]{#4}}\XS}

%\newcommand{\MA}[1][\scad]{{\taille[#1]Marc \uppercase{A}}% 
%{\sca[#1]{llain}\XS}}
\newcommand{\AuGi}[1][\scad]{\beaunom[#1]{Audrey}{G}{iremus}}

\newcommand{\AB}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc}}
\newcommand{\ABF}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc~--~Fusco}}
\newcommand{\AAB}[1][\scad]{\beaunom[#1]{Alain}{A}{bergel}}
\newcommand{\AnBa}[1][\scad]{\beaunom[#1]{Andrei}{B}{arbos}}
\newcommand{\AC}[1][\scad]{\beaunom[#1]{Alain}{C}{oulais}}
\newcommand{\AH}[1][\scad]{\beaunom[#1]{Alain}{H}{erment}}
\newcommand{\AG}[1][\scad]{\beaunom[#1]{Audrey}{G}{iremus}}
\newcommand{\AHz}[1][\scad]{\beaunom[#1]{Aurélien}{H}{azart}}
\newcommand{\AMD}[1][\scad]{\beaunom[#1]{Ali}{M}{ohammad--Djafari}}
\newcommand{\AR}[1][\scad]{\beaunom[#1]{Andrea}{R}{idolfi}}
\newcommand{\BDuc}[1][\scad]{\beaunom[#1]{Bernard}{D}{uchêne}}
\newcommand{\BH}[1][\scad]{\beaunom[#1]{Benjamin}{H}{arrou\'e}}
\newcommand{\CH}[1][\scad]{\beaunom[#1]{Christian}{H}{einrich}}
\newcommand{\CS}[1][\scad]{\beaunom[#1]{Charles}{S}{oussen}}
\newcommand{\CV}[1][\scad]{\beaunom[#1]{Cornelia}{V}{acar}}
\newcommand{\DLB}[1][\scad]{\beaunom[#1]{Denis}{L}{e Bihan}}
\newcommand{\FA}[1][\scad]{\beaunom[#1]{Frédéric}{A}{uchère}}
\newcommand{\FC}[1][\scad]{\beaunom[#1]{Frédéric}{C}{hampagnat}}
\newcommand{\FrCa}[1][\scad]{\beaunom[#1]{Fran\c{c}ois}{C}{aron}}
\newcommand{\FL}[1][\scad]{\beaunom[#1]{Franck}{L}{etimonier}}
\newcommand{\FV}[1][\scad]{\beaunom[#1]{Francisco}{V}{arela}}
\newcommand{\FDU}[1][\scad]{\beaunom[#1]{Frédéric}{D}{ublanchet}}
\newcommand{\FB}[1][\scad]{\beaunom[#1]{François}{B}{oulanger}}
\newcommand{\FO}[1][\scad]{\beaunom[#1]{Fran\c{c}ois}{O}{rieux}}
\newcommand{\GDE}[1][\scad]{\beaunom[#1]{Guy}{D}{emoment}}
\newcommand{\GS}[1][\scad]{\beaunom[#1]{Grégory}{S}{trubel}}
\newcommand{\GLB}[1][\scad]{\beaunom[#1]{Guy}{L}{e Besnerais}}
\newcommand{\GL}[1][\scad]{\beaunom[#1]{Guilaine }{L}{agache}}
\newcommand{\GR}[1][\scad]{\beaunom[#1]{Gilles}{R}{ochefort}}
\newcommand{\HC}[1][\scad]{\beaunom[#1]{Hervé}{C}{arfantan}}
\newcommand{\HS}[1][\scad]{\beaunom[#1]{Hichem}{S}{noussi}}
\newcommand{\JCV}[1][\scad]{\beaunom[#1]{Jean--Claude}{V}{ial}}
\newcommand{\JFB}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{B}{ercher}}
\newcommand{\JFG}[1][\scad]{\beaunom[#1]{Jean\,--\,Fran\c{c}ois}{G}{iovan\-nel\-li}}
\newcommand{\JFM}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{M}{angin}}
\newcommand{\JI}[1][\scad]{\beaunom[#1]{Jérôme}{I}{dier}}
\newcommand{\JeSo}[1][\scad]{\beaunom[#1]{Jessica}{S}{odjo}}
\newcommand{\JBP}[1][\scad]{\beaunom[#1]{Jean-Baptiste}{P}{oline}}
\newcommand{\KS}[1][\scad]{\beaunom[#1]{Ken}{S}{auer}}
\newcommand{\LG}[1][\scad]{\beaunom[#1]{Line}{G}{arnero}}
\newcommand{\MA}[1][\scad]{\beaunom[#1]{Marc}{A}{llain}}
\newcommand{\MF}[1][\scad]{\beaunom[#1]{Marc}{F}{ayolle}}
\newcommand{\Mimi}[1][\scad]{\beaunom[#1]{Myriam}{F}{iani}}
\newcommand{\MN}[1][\scad]{\beaunom[#1]{Mila}{N}{ikolova}}
\newcommand{\MP}[1][\scad]{\beaunom[#1]{Marcelo}{P}{ereyra}}
\newcommand{\NBA}[1][\scad]{\beaunom[#1]{Nicolas}{B}{arbey}}
\newcommand{\OF}[1][\scad]{\beaunom[#1]{Olivier}{F}{\'eron}}
\newcommand{\PC}[1][\scad]{\beaunom[#1]{Philippe}{C}{iuciu}}
\newcommand{\PG}[1][\scad]{\beaunom[#1]{Pierre}{G}{rangeat}}
\newcommand{\PS}[1][\scad]{\beaunom[#1]{Pascal}{S}{zacherski}}
\newcommand{\PM}[1][\scad]{\beaunom[#1]{Pierre}{M}{invielle}}
\newcommand{\RB}[1][\scad]{\beaunom[#1]{Redha}{B}{oubertakh}}
\newcommand{\SB}[1][\scad]{\beaunom[#1]{Stéphane}{B}{rette}}
\newcommand{\SG}[1][\scad]{\beaunom[#1]{Stéphane}{G}{autier}}
\newcommand{\SBA}[1][\scad]{\beaunom[#1]{Sylvain}{B}{ailet}}
\newcommand{\TM}[1][\scad]{\beaunom[#1]{Thierry}{M}{artin}}
\newcommand{\TR}[1][\scad]{\beaunom[#1]{Thomas}{R}{odet}}
\newcommand{\TB}[1][\scad]{\beaunom[#1]{Thomas}{B}{enoudiba}}
\newcommand{\VS}[1][\scad]{\beaunom[#1]{Vincent}{S}{amson}}
\newcommand{\YB}[1][\scad]{\beaunom[#1]{Yannick}{B}{erthoumieu}}
\newcommand{\YG}[1][\scad]{\beaunom[#1]{Yves}{G}{oussard}}



% Acronymes et raccourcis

	\def\EEA{Électronique Électrotechnique Automatique\XS}
	\newcommand{\eea}[1][\scad]{\sca[#1]{eea}\XS}

	\def\IMA{Institut de Maintenance Aéronautique\XS}
	\newcommand{\ima}[1][\scad]{\sca[#1]{ima}\XS}

	\def\EAPSI{Électronique, Automatique, Productique et Signal-Omage\XS}
	\newcommand{\eapsi}[1][\scad]{\sca[#1]{eapsi}\XS}

	\def\GSAT{Génie des Systèmes pour l'Aéronautique et les Transports\XS}
	\newcommand{\gsat}[1][\scad]{\sca[#1]{gsat}\XS}

	\def\ANR{Agence Nationale de la Recherche\XS}
	\newcommand{\anr}[1][\scad]{\sca[#1]{anr}\XS}

	\def\ENSEIRB{École Nationale Supérieure d'\'Electronique, Informatique et Télécommunications de Bordeaux\XS}
	\newcommand{\enseirb}[1][\scad]{\sca[#1]{enseirb}\XS}
	%
	\newcommand{\matmeca}[1][\scad]{\sca[#1]{matmeca}\XS}

	\def\ENSC{École Nationale Supérieure de Cognitique\XS}
	\newcommand{\ensc}[1][\scad]{\sca[#1]{ensc}\XS}

	\def\ATS{Automatique et Traitement du Signal\XS}
	\newcommand{\ats}[1][\scad]{\sca[#1]{ats}\XS}

	\def\THCS{Traitement Harmonique et Contrôle du Signal\XS}
	\newcommand{\thcs}[1][\scad]{\sca[#1]{thcs}\XS}

	\def\TE{travaux d'études\XS}
	\newcommand{\te}[1][\scad]{\sca[#1]{te}\XS}

	\def\TD{travaux dirigés\XS}
	\def\GTD{Travaux dirigés\XS}
	\newcommand{\td}[1][\scad]{\sca[#1]{td}\XS}

	\def\TP{travaux pratiques\XS}
	\def\GTP{Travaux pratiques\XS}
	\newcommand{\tp}[1][\scad]{\sca[#1]{tp}\XS}

	\def\TDAO{travaux dirigés assistés sur ordinateur\XS}
	\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}

	\def\ATER{Attaché temporaire d'enseignement et de recherche}
	\newcommand{\ater}[1][\scad]{\sca[#1]{ater}\xspace}

	\def\ADDOC{Agir pour les Doctorants et les jeunes Docteurs\XS}
	\newcommand{\addoc}[1][\scad]{\sca[#1]{addoc}\XS}

	\def\SHFJ{Service Hospitalier Frédéric Joliot\XS}
	\newcommand{\shfj}[1][\scad]{\sca[#1]{shfj}\XS}

	\def\UNAF{Unité de Neuroimagerie Anatomo Fonctionnelle\XS}
	\newcommand{\unaf}[1][\scad]{\sca[#1]{unaf}\XS}

	\def\CHU{Centre Hospitalier Universitaire\XS}
	\newcommand{\chu}[1][\scad]{\sca[#1]{chu}\XS}

	\def\LIF{Laboratoire d'Imagerie Fonctionnelle\XS}
	\newcommand{\lif}[1][\scad]{\sca[#1]{lif}\XS}

	\def\CEA{Commissariat à l'Énegie Atomique\XS}
	\newcommand{\cea}[1][\scad]{\sca[#1]{cea}\XS}

	\def\DRM{Département de Recherche Médicale\XS}
	\newcommand{\drm}[1][\scad]{\sca[#1]{drm}\XS}

	\def\DAM{Direction des Affaires Militaires\XS}
	\newcommand{\dam}[1][\scad]{\sca[#1]{dam}\XS}

	\def\DSV{Direction des Sciences du Vivant\XS}
	\newcommand{\dsv}[1][\scad]{\sca[#1]{dsv}\XS}

	\def\CNRS{Centre National de la Recherche Scientifique\XS}
	\newcommand{\cnrs}[1][\scad]{\sca[#1]{cnrs}\XS}

	\def\UMR{Unité Mixte de Recherche\XS}
	\newcommand{\umr}[1][\scad]{\sca[#1]{umr}\XS}

	\def\CNES{Centre National d'Études Spatiales\XS}
	\newcommand{\cnes}[1][\scad]{\sca[#1]{cnes}\XS}

	\def\EDF{Électricité de France\XS}
	\newcommand{\edf}[1][\scad]{\sca[#1]{edf}\XS}

	\def\ENSTA{École Nationale Supérieure de Techniques Avancées\XS}
	\newcommand{\ensta}[1][\scad]{\sca[#1]{ensta}\XS}

	\def\ENST{École Nationale Supérieure des Télécommunications\XS}
	\newcommand{\enst}[1][\scad]{\sca[#1]{enst}\XS}

	\def\ESIEA{École Supérieure d'Informatique Électronique Automatique\XS}
	\newcommand{\esiea}[1][\scad]{\sca[#1]{esiea}\XS}

	\def\ENSEA{École Nationale Supérieure de l'Électronique et des ses Applications\XS}
	\newcommand{\ensea}[1][\scad]{\sca[#1]{ensea}\XS}

	\def\GPI{Groupe Problèmes Inverses\XS}
	\newcommand{\gpi}[1][\scad]{\sca[#1]{gpi}\XS}

	\def\GSI{Groupe Signal~--~Image\XS}
	\newcommand{\gsi}[1][\scad]{\sca[#1]{gsi}\XS}

	\def\IPB{Institut Polytechnique de Bordeaux\XS}
	\newcommand{\ipb}[1][\scad]{\sca[#1]{ipb}\XS}

	\def\BINP{Bordeaux Institut National Polytechnique\XS}
	\newcommand{\binp}[1][\scad]{\sca[#1]{binp}\XS}

	\def\INSERM{Institut National pour la Santé et la Recherche Médicale\XS}
	\newcommand{\inserm}[1][\scad]{\sca[#1]{inserm}\XS}

	\def\CNAM{Conservatoire National des Arts et Métiers\XS}
	\newcommand{\cnam}[1][\scad]{\sca[#1]{cnam}\XS}

	\def\OPM{Observatoire de Paris\XS}
	\newcommand{\opm}[1][\scad]{\sca[#1]{opm}\XS}

	\def\INRIA{Institut National de Recherche et Informatique et Automatique\XS}
	\newcommand{\inria}[1][\scad]{\sca[#1]{inria}\XS}

	\def\IAS{Institut d'Astrophysique Spatiale\XS}
	\newcommand{\ias}[1][\scad]{\sca[#1]{ias}\XS}

	\def\IAP{Institut d'Astrophysique de Paris\XS}
	\newcommand{\iap}[1][\scad]{\sca[#1]{iap}\XS}

	\def\IPSN{Institut de Protection et de Sureté Nucléaire\XS}
	\newcommand{\ipsn}[1][\scad]{\sca[#1]{ipsn}\XS}

	\def\LSS{Laboratoire des Signaux et Systèmes\XS}
	\newcommand{\lss}[1][\scad]{\sca[#1]{lss}\XS}

	\def\LAPS{Laboratoire Automatique, productique, Signal\XS}
	\newcommand{\laps}[1][\scad]{\sca[#1]{laps}\XS}

	\def\LIMS{Laboratoire de l'Int\'egration du Mat\'eriau au Syst\`eme\XS}
	\def\IMS{Int\'egration du Mat\'eriau au Syst\`eme\XS}
	\newcommand{\ims}[1][\scad]{\sca[#1]{ims}\XS}

	\def\IMB{Institut de Mathématique de Bordeaux\XS}
	\newcommand{\imb}[1][\scad]{\sca[#1]{imb}\XS}

	\def\LaBRI{Laboratoire Bordelais de Recherche en Informatique\XS}
	\newcommand{\labri}[1][\scad]{\sca[#1]{labri}\XS}

	\def\LIMSI{Laboratoire d'Informatique pour la Mécanique et les Sciences de l'Ingénieur\XS}
	\newcommand{\limsi}[1][\scad]{\sca[#1]{limsi-cnrs}\XS}

	\def\ONERA{Office National d'Études et de Recherches Aérospatiales\XS}
	\newcommand{\onera}[1][\scad]{\sca[#1]{onéra}\XS}

	\def\CLS{Collecte Localisation Satellites\XS}
	\newcommand{\cls}[1][\scad]{\sca[#1]{cls}\XS}

	\def\SSL{signaux et systèmes linéaires\XS}
	\def\GSSL{Signaux et systèmes linéaires\XS}
	\newcommand{\ssl}[1][\scad]{\sca[#1]{ssl}\XS}

	\def\IFIPS{Institut de Formation des Ingénieurs de Paris-Sud\XS}
	\newcommand{\ifips}[1][\scad]{\sca[#1]{ifips}\XS}

	\def\IST{Information, Systèmes et Technologie\XS}
	\newcommand{\isp}[1][\scad]{\sca[#1]{ist}\XS}

	\def\ISC{Ingénierie des Systèmes Complexes\XS}
	\newcommand{\isc}[1][\scad]{\sca[#1]{isc}\XS}

	\def\pISIS{Ingénierie des Systèmes pour l'Image et le Signal\XS}
	\newcommand{\pisis}[1][\scad]{\sca[#1]{isis}\XS}

	\def\LMD{Licence, Master, Doctorat\XS}
	\newcommand{\lmd}[1][\scad]{\sca[#1]{lmd}\XS}

   \def\MDC{Maître de conférences\XS}
   \newcommand{\mdc}[1][\scad]{\sca[#1]{mdc}\XS}

   \def\UPS{Université Paris-Sud\XS}
   \newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}

   \def\UBI{Universit\'e Bordeaux~1\XS}
   \newcommand{\ubI}[1][\scad]{\sca[#1]{ub{\footnotesize 1}}\XS}

   \def\UdB{Universit\'e de Bordeaux\XS}
   \newcommand{\udb}[1][\scad]{\sca[#1]{ub}\XS}

   \def\TdSI{Traitement du Signal et de l'Image\XS}
   \newcommand{\tdsi}[1][\scad]{\sca[#1]{tdsi}\XS}

   \def\SDI{Sciences de l'Ingénieur\XS}
   \newcommand{\sdi}[1][\scad]{\sca[#1]{sdi}\XS}



% Unites Thomson
   %\newcommand{\thomair}[1][\scad]{\sca[#1]{Thomson-csf Airsys}\XS}
   %\newcommand{\oscar}[1][\scad]{\sca[#1]{Oscar}\XS}
   %\newcommand{\thomrcm}[1][\scad]{\sca[#1]{Thomson-rcm}\XS}

% Divers à virer...
   % LENA, lena upr640,...
   %\newcommand{\uprlen}[1][\scad]{\sca[#1]{upr}{\footnotesize 640}\XS}
   %\def\LENA{Laboratoire d'Encéphalographie et de Neurophysiologie Appliquée\XS}
   %\newcommand{\lena}[1][\scad]{\sca[#1]{lena}\XS}

   %\newcommand{\UFRPhys}[1][\scad]{{\ufr de physique}\XS}
   %\newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}




==> alphabet.tex <==
% Document LaTeX        Auteur : Guy Le Besnerais       Date : 25/05/94
% Modification : J.-F. Gio      (15/09/95)
%                               J.I. (format Latex 2e, taille adaptative 22/03/99)
%                                    (fonte blackboard 27/08/99)
%
% ==> OK, JFG -- 26/04/2010
%
% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace, amsmath, bbm)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}
%\RequirePackage{bbm}
\RequirePackage{dsfont}
\RequirePackage{oldgerm}		% 04.06.2003   Pour les alphabet Gothiques

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif

%\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)
\def\sbl#1{\ensuremath{\mathds{#1}}}              % Style blackboard (necessite bbm)

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{v}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}

% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\varkappab   {{\sbmm{\varkappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}     \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}         \def\Xib       {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}         \def\Pib       {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}   \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib      {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib      {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}   \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}

\def\ellb{{\sbmm{\ell}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}
\def\eK{\Kbb}

% ALPHABET GOTHIQUES  04.06.2003  M.M. ICHIR

\def\Ag{{\textgoth{A}}\XS}  \def\ag{{\textgoth{a}}\XS}
\def\Bg{{\textgoth{B}}\XS}  \def\bg{{\textgoth{b}}\XS}
\def\Cg{{\textgoth{C}}\XS}  \def\cg{{\textgoth{c}}\XS}
\def\Dg{{\textgoth{D}}\XS}  \def\dg{{\textgoth{d}}\XS}
\def\Eg{{\textgoth{E}}\XS}  \def\eg{{\textgoth{e}}\XS}
\def\Fg{{\textgoth{F}}\XS}  \def\fg{{\textgoth{f}}\XS}
\def\Gg{{\textgoth{G}}\XS}  %\def\gg{{\textgoth{g}}\XS}
\def\Hg{{\textgoth{H}}\XS}  \def\hg{{\textgoth{h}}\XS}
\def\Ig{{\textgoth{I}}\XS}  \def\ig{{\textgoth{i}}\XS}
\def\Jg{{\textgoth{J}}\XS}  \def\jg{{\textgoth{j}}\XS}
\def\Kg{{\textgoth{K}}\XS}  \def\kg{{\textgoth{k}}\XS}
\def\Lg{{\textgoth{L}}\XS}  \def\lg{{\textgoth{l}}\XS}
\def\Mg{{\textgoth{M}}\XS}  \def\mg{{\textgoth{m}}\XS}
\def\Ng{{\textgoth{N}}\XS}  \def\ng{{\textgoth{n}}\XS}
\def\Og{{\textgoth{O}}\XS}  \def\og{{\textgoth{o}}\XS}
\def\Pg{{\textgoth{P}}\XS}  \def\pg{{\textgoth{p}}\XS}
\def\Qg{{\textgoth{Q}}\XS}  \def\qg{{\textgoth{q}}\XS}
\def\Rg{{\textgoth{R}}\XS}  \def\rg{{\textgoth{r}}\XS}
\def\Sg{{\textgoth{S}}\XS}  \def\sg{{\textgoth{s}}\XS}
\def\Tg{{\textgoth{T}}\XS}  \def\tg{{\textgoth{t}}\XS}
\def\Ug{{\textgoth{U}}\XS}  \def\ug{{\textgoth{u}}\XS}
\def\Vg{{\textgoth{V}}\XS}  \def\vg{{\textgoth{v}}\XS}
\def\Wg{{\textgoth{W}}\XS}  \def\wg{{\textgoth{w}}\XS}
\def\Xg{{\textgoth{X}}\XS}  \def\xg{{\textgoth{x}}\XS}
\def\Yg{{\textgoth{Y}}\XS}  \def\yg{{\textgoth{y}}\XS}
\def\Zg{{\textgoth{Z}}\XS}  \def\zg{{\textgoth{z}}\XS}

